Supervised and Extended Restart in Random Walks for Ranking and Link Prediction in Networks

Given a real-world graph, how can we measure relevance scores for ranking and link prediction? Random walk with restart (RWR) provides an excellent measure for this and has been applied to various applications such as friend recommendation, community detection, anomaly detection, etc. However, RWR suffers from two problems: 1) using the same restart probability for all the nodes limits the expressiveness of random walk, and 2) the restart probability needs to be manually chosen for each application without theoretical justification. We have two main contributions in this paper. First, we propose Random Walk with Extended Restart (RWER), a random walk based measure which improves the expressiveness of random walks by using a distinct restart probability for each node. The improved expressiveness leads to superior accuracy for ranking and link prediction. Second, we propose SuRe (Supervised Restart for RWER), an algorithm for learning the restart probabilities of RWER from a given graph. SuRe eliminates the need to heuristically and manually select the restart parameter for RWER. Extensive experiments show that our proposed method provides the best performance for ranking and link prediction tasks, improving the MAP (Mean Average Precision) by up to 15.8% on the best competitor.

==> 070journal.tex <==
\begin{algorithm} [t!]
	\small
	\begin{algorithmic}[1]
		\caption{\sure-F \space- Fast algorithm for learning a restart vector $\cc$} \label{alg:learning:restart_fast}
		\REQUIRE adjacency matrix $\A$, query node $s$, positive node set $P$, negative node set $N$, origin vector $\oo$, parameter $b$ of loss function $h$, and the learning rate $\eta$
		\ENSURE the learned restart vector $\cc$
		\STATE initialize $\cc \leftarrow \oo$
		\WHILE {not converged}
		\STATE compute $\rr$
		\STATE initialize $\vect{p}$ such that $p_x= \sum_{y\in N}\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}, p_y =\sum_{x \in P}-\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}$ for all $x \in P, y \in N$, and the others are $0$.
		%        \STATE compute $\rr$
		%        \STATE compute $\frac{\partial r_x}{\partial \cc}$ and $\frac{\partial r_y}{\partial \cc} (\forall x \in P, \forall y \in N)$ by Eq.~\eqref{eq:deriv_r}
	%		\STATE compute $\frac{\partial r_x}{\partial \cc}$ and $\frac{\partial r_y}{\partial \cc}$ by equations~\eqref{eq:deriv_r}~and~\eqref{eq:deriv_r2}\label{alg:method:sure:partial}
		\STATE compute $\sum_{x\in P, y\in N} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}} (\frac{\partial r_y}{\partial \cc} - \frac{\partial r_x}{\partial \cc} )$ by equation~\eqref{eq:journal:drdc} \label{alg:fast:sure:vector}
	
		\STATE compute $\frac{\partial F(\cc)}{\partial \cc}$ by equation~\eqref{eq:deriv_obj} \label{alg:fast:restart:obj}
		\STATE update $\cc \leftarrow \cc - \eta \frac{\partial F(\cc)}{\partial \cc}$ \label{alg:fast:restart:update}
		\ENDWHILE
		\RETURN $\cc$
	\end{algorithmic}
\end{algorithm}


\begin{equation}
\label{eq:new_deriv_r}
%    \small
\frac{\partial r_x}{\partial \cc} = \frac{\partial M(x,s)}{\partial \cc} = \nA \left( M(x,s) \vect{1} - \MM(x,:)^\top \right)^\top \circ \MM(:,s)
\end{equation}

Using the equation~\eqref{eq:deriv_r} and \eqref{eq:deriv_r2}, $\sum_{x\in P, y\in N}\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}} (\frac{\partial r_y}{\partial \cc} - \frac{\partial r_x}{\partial \cc} )$ is represented as follows:
\begin{equation}
\label{eq:journal:drdc}
\small
\left((-\nA^\top + \mat{e}_s \mat{1}^\top )^\top \sum_{x, y} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top \right ) \circ \MM(:,s)
\end{equation}
where $\vect{M}$ is $(\mat{I} -\nA^\top (\mat{I} - diag(\cc) ) + \qq (\cc - \mat{1})^\top)^{-1}$
%$ \left((-\nA^\top + \mat{e}_s \mat{1}^\top )^\top \sum_{x, y} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top \right ) \circ \MM(:,s)$


\begin{lemma}
	\label{lemma:journal:drdc}
	In equation~\eqref{eq:journal:drdc}, $\sum_{x, y} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top$ is represented as $\mat{M}^\top \vect{p}$ where $\vect{p}(x)= \sum_{y\in N}\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}, \vect{p}(y) =\sum_{x \in P}-\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}$, and all other elements of $\vect{p}$ is $0$. 
	The computation of $\sum_{x, y} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top$ takes $O(Tm+|P||N|)$ time.
%	Suppose $\sum_{x\in P, y\in N} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}} (\frac{\partial r_y}{\partial \cc} - \frac{\partial r_x}{\partial \cc} )$ is $\tilde{\rr}$. 
%	Then, $\tilde{\rr}$ is $\mat{M}^\top \vect{p}$, where $\mat{M} = (\mat{I} - \nA^\top (\mat{I} - diag(\cc) ) + \qq (\cc - \mat{1})^\top)^{-1} $, and $\vect{p}(x)= \sum_{y\in N}\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}, \vect{p}(y) =\sum_{x \in P}-\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}$, and the other elements of $\vect{p}$ is $0$. 
%	Also, time complexity of computing $\tilde{\rr}$ iteratively (Lemma~\ref{lemma:method:Mx}) is $O(Tm)$ where $T$ is the number of iterations for computing $\tilde{\rr}$, and $m$ is the number of edges.
	\begin{proof}		
		To simplify the proof, we only consider one $(x,y)$ pair.
		According to Lemma~\ref{lemma:method:Mx}, $\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}\MM(x,:)^\top$ is $\MM^\top \vect{p}$, where $\vect{p}(x)=\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}$ and other elements are $0$.
		Similarly, we can compute  $\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}\MM(y,:)$.
		Hence $ \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top$ is $\MM^\top \vect{p}$, where $\vect{p}(y)=\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}, \vect{p}(x)=-\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}$  and other elements are $0$.
		 $\vect{p}(x)= \sum_{y\in N}\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}, \vect{p}(y) =\sum_{x \in P}-\frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}$.
		
%		 $\tilde{\rr}=\sum_{x\in P, y\in N} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top= \MM^\top \vect{p}$
		Initializing $\vect{p}$ takes $O(|P||N|)$ time. 
		By Lemma~\ref{lemma:method:derivtime}, computing $\sum_{x\in P, y\in N} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top$ iteratively takes $O(Tm)$ time, where $T$ is the number of iterations for computing $\tilde{\rr}$, and $m$ is the number of edges.
		Hence, overall time for computing $\sum_{x, y} \frac{\partial h(\delta_{yx})}{\partial \delta_{yx}}(\MM(y,:)-\MM(x,:))^\top$ is $O(Tm+|P||N|)$.

	\end{proof}
\end{lemma}
